Characterization of a vacuum ultraviolet light source at 118 nm

Vacuum ultraviolet (VUV) light at 118 nm has been shown to be a powerful tool to ionize molecules for various gas-phase chemical studies. A convenient table top source of 118 nm light can be produced by frequency tripling 355 nm light from a Nd:YAG laser in xenon gas. This process has a low efficiency, typically producing only nJ/pulse of VUV light. Simple models of the tripling process predict the power of 118 nm light produced should increase quadratically with increasing xenon pressure. However, experimental 118 nm production has been observed to reach a maximum and then decrease to zero with increasing xenon pressure. Here, we describe the basic theory and experimental setup for producing 118 nm light and a new proposed model for the mechanism limiting the production based on pressure broadened absorption.

==> 118paper_bib.tex <==
%%% NIST webbook
@Misc{NIST_ASD,
author = {A.~Kramida and {Yu.~Ralchenko} and
J.~Reader and {and NIST ASD Team}},
HOWPUBLISHED = {{NIST Atomic Spectra Database
(ver. 5.3), [Online]. Available:
{\tt{http://physics.nist.gov/asd}} [2016, January 29].
National Institute of Standards and Technology,
Gaithersburg, MD.}},
year = {2015},
}


%%%% SFG and other nonlinear things

@article{Bethune1976,
  title = {Optical Quadrupole Sum-Frequency Generation in Sodium Vapor},
  author = {Bethune, D. S. and Smith, R. W. and Shen, Y. R.},
  journal = {Phys. Rev. Lett.},
  volume = {37},
  issue = {7},
  pages = {431--434},
  numpages = {0},
  year = {1976},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.37.431},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.37.431}
}

@article{Bethune1978,
  title = {Sum-frequency generation via a resonant quadrupole transition in sodium},
  author = {Bethune, Donald S. and Smith, Robert W. and Shen, Y. R.},
  journal = {Phys. Rev. A},
  volume = {17},
  issue = {1},
  pages = {277--292},
  numpages = {0},
  year = {1978},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.17.277},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.17.277}
}


@article{Bethune1981,
  title = {Optical second-harmonic generation in atomic vapors with focused beams},
  author = {Bethune, D. S.},
  journal = {Phys. Rev. A},
  volume = {23},
  issue = {6},
  pages = {3139--3151},
  numpages = {0},
  year = {1981},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.23.3139},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.23.3139}
}


@article{Finn1971,
  title = {dc-Induced Optical Second-Harmonic Generation in the Inert Gases},
  author = {Finn, R. S. and Ward, J. F.},
  journal = {Phys. Rev. Lett.},
  volume = {26},
  issue = {6},
  pages = {285--289},
  numpages = {0},
  year = {1971},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.26.285},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.26.285}
}


@article{Flusberg1977,
  title = {Optical Difference-Frequency Generation in Atomic Thallium Vapor},
  author = {Flusberg, A. and Mossberg, T. and Hartmann, S. R.},
  journal = {Phys. Rev. Lett.},
  volume = {38},
  issue = {2},
  pages = {59--62},
  numpages = {0},
  year = {1977},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.38.59},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.38.59}
}

@article{Jamroz1982, 
author = {W. Jamroz and P. E. LaRocque and B. P. Stoicheff}, 
journal = {Opt. Lett.}, 
keywords = {},
number = {4}, 
pages = {148--150}, 
publisher = {OSA},
title = {Resonantly enhanced second-harmonic generation in zinc vapor}, 
volume = {7}, 
month = {Apr},
year = {1982},
url = {http://ol.osa.org/abstract.cfm?URI=ol-7-4-148},
doi = {10.1364/OL.7.000148},
}

@article{Malcuit1990,
  title = {Anomalies in optical harmonic generation using high-intensity laser radiation},
  author = {Malcuit, Michelle S. and Boyd, Robert W. and Davis, William V. and Rza\ifmmode \mbox{\c{}}\else \c{}\fi{}ewski, Kazimierz},
  journal = {Phys. Rev. A},
  volume = {41},
  issue = {7},
  pages = {3822--3825},
  numpages = {0},
  year = {1990},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.41.3822},
  url = {http://link.aps.org/doi/10.1103/PhysRevA.41.3822}
}

@article{Marmet1992, 
author = {L. Marmet and K. Hakuta and B. P. Stoicheff}, 
journal = {J. Opt. Soc. Am. B}, 
keywords = {},
number = {7}, 
pages = {1038--1046}, 
publisher = {OSA},
title = {Second-harmonic generation in atomic hydrogen induced by a charge-separation field}, 
volume = {9}, 
month = {Jul},
year = {1992},
url = {http://josab.osa.org/abstract.cfm?URI=josab-9-7-1038},
doi = {10.1364/JOSAB.9.001038}
}

@article{Matsuoka1977,
  title = {Optical Second-Harmonic Generation in Gases: "Rotation" of Quadrupole Moment in Magnetic Field},
  author = {Matsuoka, M. and Nakatsuka, H. and Uchiki, H. and Mitsunaga, M.},
  journal = {Phys. Rev. Lett.},
  volume = {38},
  issue = {16},
  pages = {894--898},
  numpages = {0},
  year = {1977},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.38.894},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.38.894}
}

@article{Miyazaki1979,
  title = {Spontaneous-Field-Induced Optical Second-Harmonic Generation in Atomic Vapors},
  author = {Miyazaki, Kenzo and Sato, Takuzo and Kashiwagi, Hiroshi},
  journal = {Phys. Rev. Lett.},
  volume = {43},
  issue = {16},
  pages = {1154--1157},
  numpages = {0},
  year = {1979},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.43.1154},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.43.1154}
}

@article{Mossberg1978,
title = "Optical second-harmonic generation in atomic thallium vapor",
journal = "Optics Communications",
volume = "25",
number = "1",
pages = "121 - 124",
year = "1978",
note = "",
issn = "0030-4018",
doi = "http://dx.doi.org/10.1016/0030-4018(78)90104-9",
url = "http://www.sciencedirect.com/science/article/pii/0030401878901049",
author = "T. Mossberg and A. Flusberg and S.R. Hartmann",

}
@article{Shi2009,
   author = "Shi, Y. J. and Al-Basheer, W. and Thompson, R. I.",
   title = "Two-photon resonant second harmonic generation in atomic xeon",
   journal = "The Journal of Chemical Physics",
   year = "2009",
   volume = "130",
   number = "9", 
   eid = 094305,
   pages = "",
   url = "http://scitation.aip.org/content/aip/journal/jcp/130/9/10.1063/1.3079617",
   doi = "http://dx.doi.org/10.1063/1.3079617" 
}

@article{Ferrell1987,
  title = {Resonance broadening and shifting of spectral lines in xenon and krypton},
  author = {Ferrell, Wanda R. and Payne, M. G. and Garrett, W. R.},
  journal = {Phys. Rev. A},
  volume = {36},
  issue = {1},
  pages = {81--89},
  numpages = {0},
  year = {1987},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.36.81},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.36.81}
}

@article{Chan1992,
  title = {Absolute optical oscillator strengths for the electronic excitation of atoms at high resolution. II. The photoabsorption of neon},
  author = {Chan, W. F. and Cooper, G. and Guo, X. and Brion, C. E.},
  journal = {Phys. Rev. A},
  volume = {45},
  issue = {3},
  pages = {1420--1433},
  numpages = {0},
  year = {1992},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.45.1420},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.45.1420}
}
